Adaptive Neural Ranking Framework: Toward Maximized Business Goal for Cascade Ranking Systems

Cascade ranking is widely used for large-scale top-k selection problems in online advertising and recommendation systems, and learning-to-rank is an important way to optimize the models in cascade ranking. Previous works on learning-to-rank usually focus on letting the model learn the complete order or top-k order, and adopt the corresponding rank metrics (e.g. OPA and NDCG@k) as optimization targets. However, these targets can not adapt to various cascade ranking scenarios with varying data complexities and model capabilities; and the existing metric-driven methods such as the Lambda framework can only optimize a rough upper bound of limited metrics, potentially resulting in sub-optimal and performance misalignment. To address these issues, we propose a novel perspective on optimizing cascade ranking systems by highlighting the adaptability of optimization targets to data complexities and model capabilities. Concretely, we employ multi-task learning to adaptively combine the optimization of relaxed and full targets, which refers to metrics Recall@m@k and OPA respectively. We also introduce permutation matrix to represent the rank metrics and employ differentiable sorting techniques to relax hard permutation matrix with controllable approximate error bound. This enables us to optimize both the relaxed and full targets directly and more appropriately. We named this method as Adaptive Neural Ranking Framework (abbreviated as ARF). Furthermore, we give a specific practice under ARF. We use the NeuralSort to obtain the relaxed permutation matrix and draw on the variant of the uncertainty weight method in multi-task learning to optimize the proposed losses jointly. Experiments on a total of 4 public and industrial benchmarks show the effectiveness and generalization of our method, and online experiment shows that our method has significant application value.

==> bib_backup.tex <==
@inproceedings{LambdaFramework2018,
  author       = {Xuanhui Wang and
                  Cheng Li and
                  Nadav Golbandi and
                  Michael Bendersky and
                  Marc Najork},
  title        = {The LambdaLoss Framework for Ranking Metric Optimization},
  booktitle    = {Proceedings of the 27th {ACM} International Conference on Information
                  and Knowledge Management, {CIKM} 2018, Torino, Italy, October 22-26,
                  2018},
  pages        = {1313--1322},
  publisher    = {{ACM}},
  year         = {2018},
  url          = {https://doi.org/10.1145/3269206.3271784},
  doi          = {10.1145/3269206.3271784},
  timestamp    = {Tue, 29 Dec 2020 18:42:42 +0100},
  biburl       = {https://dblp.org/rec/conf/cikm/WangLGBN18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pirank2021,
  author       = {Robin M. E. Swezey and
                  Aditya Grover and
                  Bruno Charron and
                  Stefano Ermon},
  title        = {PiRank: Scalable Learning To Rank via Differentiable Sorting},
  booktitle    = {Advances in Neural Information Processing Systems 34: Annual Conference
                  on Neural Information Processing Systems 2021, NeurIPS 2021, December
                  6-14, 2021, virtual},
  pages        = {21644--21654},
  year         = {2021},
  url          = {https://proceedings.neurips.cc/paper/2021/hash/b5200c6107fc3d41d19a2b66835c3974-Abstract.html},
  timestamp    = {Tue, 03 May 2022 16:20:49 +0200},
  biburl       = {https://dblp.org/rec/conf/nips/SwezeyGCE21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{neuralsort2019,
  author       = {Aditya Grover and
                  Eric Wang and
                  Aaron Zweig and
                  Stefano Ermon},
  title        = {Stochastic Optimization of Sorting Networks via Continuous Relaxations},
  booktitle    = {7th International Conference on Learning Representations, {ICLR} 2019,
                  New Orleans, LA, USA, May 6-9, 2019},
  publisher    = {OpenReview.net},
  year         = {2019},
  url          = {https://openreview.net/forum?id=H1eSS3CcKX},
  timestamp    = {Thu, 25 Jul 2019 14:25:45 +0200},
  biburl       = {https://dblp.org/rec/conf/iclr/GroverWZE19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{tfranking2019,
  author       = {Rama Kumar Pasumarthi and
                  Sebastian Bruch and
                  Xuanhui Wang and
                  Cheng Li and
                  Michael Bendersky and
                  Marc Najork and
                  Jan Pfeifer and
                  Nadav Golbandi and
                  Rohan Anil and
                  Stephan Wolf},
  title        = {TF-Ranking: Scalable TensorFlow Library for Learning-to-Rank},
  booktitle    = {Proceedings of the 25th {ACM} {SIGKDD} International Conference on
                  Knowledge Discovery {\&} Data Mining, {KDD} 2019, Anchorage, AK,
                  USA, August 4-8, 2019},
  pages        = {2970--2978},
  publisher    = {{ACM}},
  year         = {2019},
  url          = {https://doi.org/10.1145/3292500.3330677},
  doi          = {10.1145/3292500.3330677},
  timestamp    = {Sun, 06 Aug 2023 20:52:17 +0200},
  biburl       = {https://dblp.org/rec/conf/kdd/PasumarthiBWLBN19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{approxNdcg2010,
  author       = {Tao Qin and
                  Tie{-}Yan Liu and
                  Hang Li},
  title        = {A general approximation framework for direct optimization of information
                  retrieval measures},
  journal      = {Inf. Retr.},
  volume       = {13},
  number       = {4},
  pages        = {375--397},
  year         = {2010},
  url          = {https://doi.org/10.1007/s10791-009-9124-x},
  doi          = {10.1007/s10791-009-9124-x},
  timestamp    = {Wed, 04 Jul 2018 12:02:34 +0200},
  biburl       = {https://dblp.org/rec/journals/ir/QinLL10.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ranknet2005,
  author       = {Christopher J. C. Burges and
                  Tal Shaked and
                  Erin Renshaw and
                  Ari Lazier and
                  Matt Deeds and
                  Nicole Hamilton and
                  Gregory N. Hullender},
  title        = {Learning to rank using gradient descent},
  booktitle    = {Machine Learning, Proceedings of the Twenty-Second International Conference
                  {(ICML} 2005), Bonn, Germany, August 7-11, 2005},
  series       = {{ACM} International Conference Proceeding Series},
  volume       = {119},
  pages        = {89--96},
  publisher    = {{ACM}},
  year         = {2005},
  url          = {https://doi.org/10.1145/1102351.1102363},
  doi          = {10.1145/1102351.1102363},
  timestamp    = {Wed, 28 Nov 2018 12:57:16 +0100},
  biburl       = {https://dblp.org/rec/conf/icml/BurgesSRLDHH05.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{lambdaMart2010,
  title={From ranknet to lambdarank to lambdamart: An overview},
  author={Burges, Christopher JC},
  journal={Learning},
  volume={11},
  number={23-581},
  pages={81},
  year={2010}
}

@inproceedings{pointwise2006,
  author       = {David Cossock and
                  Tong Zhang},
  title        = {Subset Ranking Using Regression},
  booktitle    = {Learning Theory, 19th Annual Conference on Learning Theory, {COLT}
                  2006, Pittsburgh, PA, USA, June 22-25, 2006, Proceedings},
  series       = {Lecture Notes in Computer Science},
  volume       = {4005},
  pages        = {605--619},
  publisher    = {Springer},
  year         = {2006},
  url          = {https://doi.org/10.1007/11776420\_44},
  doi          = {10.1007/11776420\_44},
  timestamp    = {Fri, 08 Sep 2023 21:18:17 +0200},
  biburl       = {https://dblp.org/rec/conf/colt/CossockZ06.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pointwise2007,
  author       = {Ping Li and
                  Christopher J. C. Burges and
                  Qiang Wu},
  title        = {McRank: Learning to Rank Using Multiple Classification and Gradient
                  Boosting},
  booktitle    = {Advances in Neural Information Processing Systems 20, Proceedings
                  of the Twenty-First Annual Conference on Neural Information Processing
                  Systems, Vancouver, British Columbia, Canada, December 3-6, 2007},
  pages        = {897--904},
  publisher    = {Curran Associates, Inc.},
  year         = {2007},
  url          = {https://proceedings.neurips.cc/paper/2007/hash/b86e8d03fe992d1b0e19656875ee557c-Abstract.html},
  timestamp    = {Mon, 16 May 2022 15:41:51 +0200},
  biburl       = {https://dblp.org/rec/conf/nips/LiBW07.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pointwise2001,
  author       = {Koby Crammer and
                  Yoram Singer},
  editor       = {Thomas G. Dietterich and
                  Suzanna Becker and
                  Zoubin Ghahramani},
  title        = {Pranking with Ranking},
  booktitle    = {Advances in Neural Information Processing Systems 14 [Neural Information
                  Processing Systems: Natural and Synthetic, {NIPS} 2001, December 3-8,
                  2001, Vancouver, British Columbia, Canada]},
  pages        = {641--647},
  publisher    = {{MIT} Press},
  year         = {2001},
  url          = {https://proceedings.neurips.cc/paper/2001/hash/5531a5834816222280f20d1ef9e95f69-Abstract.html},
  timestamp    = {Mon, 16 May 2022 15:41:51 +0200},
  biburl       = {https://dblp.org/rec/conf/nips/CrammerS01.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{lts,
  author       = {Jian Yang and
                  Juncheng Wan and
                  Shuming Ma and
                  Haoyang Huang and
                  Dongdong Zhang and
                  Yong Yu and
                  Zhoujun Li and
                  Furu Wei},
  editor       = {Lu Wang and
                  Yansong Feng and
                  Yu Hong and
                  Ruifang He},
  title        = {Learning to Select Relevant Knowledge for Neural Machine Translation},
  booktitle    = {Natural Language Processing and Chinese Computing - 10th {CCF} International
                  Conference, {NLPCC} 2021, Qingdao, China, October 13-17, 2021, Proceedings,
                  Part {I}},
  series       = {Lecture Notes in Computer Science},
  volume       = {13028},
  pages        = {79--91},
  publisher    = {Springer},
  year         = {2021},
  url          = {https://doi.org/10.1007/978-3-030-88480-2\_7},
  doi          = {10.1007/978-3-030-88480-2\_7},
  timestamp    = {Wed, 19 Apr 2023 16:32:40 +0200},
  biburl       = {https://dblp.org/rec/conf/nlpcc/YangWMHZYLW21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{pointwise2002,
  author       = {Amnon Shashua and
                  Anat Levin},
  editor       = {Suzanna Becker and
                  Sebastian Thrun and
                  Klaus Obermayer},
  title        = {Ranking with Large Margin Principle: Two Approaches},
  booktitle    = {Advances in Neural Information Processing Systems 15 [Neural Information
                  Processing Systems, {NIPS} 2002, December 9-14, 2002, Vancouver, British
                  Columbia, Canada]},
  pages        = {937--944},
  publisher    = {{MIT} Press},
  year         = {2002},
  url          = {https://proceedings.neurips.cc/paper/2002/hash/51de85ddd068f0bc787691d356176df9-Abstract.html},
  timestamp    = {Mon, 16 May 2022 15:41:51 +0200},
  biburl       = {https://dblp.org/rec/conf/nips/ShashuaL02.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pairwiseBoosting1998,
  author       = {Yoav Freund and
                  Raj D. Iyer and
                  Robert E. Schapire and
                  Yoram Singer},
  editor       = {Jude W. Shavlik},
  title        = {An Efficient Boosting Algorithm for Combining Preferences},
  booktitle    = {Proceedings of the Fifteenth International Conference on Machine Learning
                  {(ICML} 1998), Madison, Wisconsin, USA, July 24-27, 1998},
  pages        = {170--178},
  publisher    = {Morgan Kaufmann},
  year         = {1998},
  timestamp    = {Thu, 30 Jun 2011 10:34:12 +0200},
  biburl       = {https://dblp.org/rec/conf/icml/FreundISS98.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pairwiseGradient2005,
  author       = {Christopher J. C. Burges and
                  Tal Shaked and
                  Erin Renshaw and
                  Ari Lazier and
                  Matt Deeds and
                  Nicole Hamilton and
                  Gregory N. Hullender},
  editor       = {Luc De Raedt and
                  Stefan Wrobel},
  title        = {Learning to rank using gradient descent},
  booktitle    = {Machine Learning, Proceedings of the Twenty-Second International Conference
                  {(ICML} 2005), Bonn, Germany, August 7-11, 2005},
  series       = {{ACM} International Conference Proceeding Series},
  volume       = {119},
  pages        = {89--96},
  publisher    = {{ACM}},
  year         = {2005},
  url          = {https://doi.org/10.1145/1102351.1102363},
  doi          = {10.1145/1102351.1102363},
  timestamp    = {Wed, 28 Nov 2018 12:57:16 +0100},
  biburl       = {https://dblp.org/rec/conf/icml/BurgesSRLDHH05.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pairwiseBoosting2007,
  author       = {Zhaohui Zheng and
                  Hongyuan Zha and
                  Tong Zhang and
                  Olivier Chapelle and
                  Keke Chen and
                  Gordon Sun},
  editor       = {John C. Platt and
                  Daphne Koller and
                  Yoram Singer and
                  Sam T. Roweis},
  title        = {A General Boosting Method and its Application to Learning Ranking
                  Functions for Web Search},
  booktitle    = {Advances in Neural Information Processing Systems 20, Proceedings
                  of the Twenty-First Annual Conference on Neural Information Processing
                  Systems, Vancouver, British Columbia, Canada, December 3-6, 2007},
  pages        = {1697--1704},
  publisher    = {Curran Associates, Inc.},
  year         = {2007},
  url          = {https://proceedings.neurips.cc/paper/2007/hash/8d317bdcf4aafcfc22149d77babee96d-Abstract.html},
  timestamp    = {Mon, 16 May 2022 15:41:51 +0200},
  biburl       = {https://dblp.org/rec/conf/nips/ZhengZZCCS07.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pairwiseSVM2006,
  author       = {Yunbo Cao and
                  Jun Xu and
                  Tie{-}Yan Liu and
                  Hang Li and
                  Yalou Huang and
                  Hsiao{-}Wuen Hon},
  editor       = {Efthimis N. Efthimiadis and
                  Susan T. Dumais and
                  David Hawking and
                  Kalervo J{\"{a}}rvelin},
  title        = {Adapting ranking {SVM} to document retrieval},
  booktitle    = {{SIGIR} 2006: Proceedings of the 29th Annual International {ACM} {SIGIR}
                  Conference on Research and Development in Information Retrieval, Seattle,
                  Washington, USA, August 6-11, 2006},
  pages        = {186--193},
  publisher    = {{ACM}},
  year         = {2006},
  url          = {https://doi.org/10.1145/1148170.1148205},
  doi          = {10.1145/1148170.1148205},
  timestamp    = {Sun, 02 Oct 2022 16:15:14 +0200},
  biburl       = {https://dblp.org/rec/conf/sigir/CaoXLLHH06.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pairwiseNonsmooth2006,
  author       = {Christopher J. C. Burges and
                  Robert Ragno and
                  Quoc Viet Le},
  editor       = {Bernhard Sch{\"{o}}lkopf and
                  John C. Platt and
                  Thomas Hofmann},
  title        = {Learning to Rank with Nonsmooth Cost Functions},
  booktitle    = {Advances in Neural Information Processing Systems 19, Proceedings
                  of the Twentieth Annual Conference on Neural Information Processing
                  Systems, Vancouver, British Columbia, Canada, December 4-7, 2006},
  pages        = {193--200},
  publisher    = {{MIT} Press},
  year         = {2006},
  url          = {https://proceedings.neurips.cc/paper/2006/hash/af44c4c56f385c43f2529f9b1b018f6a-Abstract.html},
  timestamp    = {Mon, 16 May 2022 15:41:51 +0200},
  biburl       = {https://dblp.org/rec/conf/nips/BurgesRL06.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pairwiseSoomthingDCG2009,
  author       = {Mingrui Wu and
                  Yi Chang and
                  Zhaohui Zheng and
                  Hongyuan Zha},
  editor       = {David Wai{-}Lok Cheung and
                  Il{-}Yeol Song and
                  Wesley W. Chu and
                  Xiaohua Hu and
                  Jimmy Lin},
  title        = {Smoothing {DCG} for learning to rank: a novel approach using smoothed
                  hinge functions},
  booktitle    = {Proceedings of the 18th {ACM} Conference on Information and Knowledge
                  Management, {CIKM} 2009, Hong Kong, China, November 2-6, 2009},
  pages        = {1923--1926},
  publisher    = {{ACM}},
  year         = {2009},
  url          = {https://doi.org/10.1145/1645953.1646266},
  doi          = {10.1145/1645953.1646266},
  timestamp    = {Sun, 02 Oct 2022 15:57:20 +0200},
  biburl       = {https://dblp.org/rec/conf/cikm/WuCZZ09.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{listwise2007,
  author       = {Zhe Cao and
                  Tao Qin and
                  Tie{-}Yan Liu and
                  Ming{-}Feng Tsai and
                  Hang Li},
  editor       = {Zoubin Ghahramani},
  title        = {Learning to rank: from pairwise approach to listwise approach},
  booktitle    = {Machine Learning, Proceedings of the Twenty-Fourth International Conference
                  {(ICML} 2007), Corvallis, Oregon, USA, June 20-24, 2007},
  series       = {{ACM} International Conference Proceeding Series},
  volume       = {227},
  pages        = {129--136},
  publisher    = {{ACM}},
  year         = {2007},
  url          = {https://doi.org/10.1145/1273496.1273513},
  doi          = {10.1145/1273496.1273513},
  timestamp    = {Tue, 06 Nov 2018 16:58:29 +0100},
  biburl       = {https://dblp.org/rec/conf/icml/CaoQLTL07.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{listwise2008,
  author       = {Fen Xia and
                  Tie{-}Yan Liu and
                  Jue Wang and
                  Wensheng Zhang and
                  Hang Li},
  editor       = {William W. Cohen and
                  Andrew McCallum and
                  Sam T. Roweis},
  title        = {Listwise approach to learning to rank: theory and algorithm},
  booktitle    = {Machine Learning, Proceedings of the Twenty-Fifth International Conference
                  {(ICML} 2008), Helsinki, Finland, June 5-9, 2008},
  series       = {{ACM} International Conference Proceeding Series},
  volume       = {307},
  pages        = {1192--1199},
  publisher    = {{ACM}},
  year         = {2008},
  url          = {https://doi.org/10.1145/1390156.1390306},
  doi          = {10.1145/1390156.1390306},
  timestamp    = {Tue, 06 Nov 2018 16:58:28 +0100},
  biburl       = {https://dblp.org/rec/conf/icml/XiaLWZL08.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{listwiseAdaRank2007,
  author       = {Jun Xu and
                  Hang Li},
  editor       = {Wessel Kraaij and
                  Arjen P. de Vries and
                  Charles L. A. Clarke and
                  Norbert Fuhr and
                  Noriko Kando},
  title        = {AdaRank: a boosting algorithm for information retrieval},
  booktitle    = {{SIGIR} 2007: Proceedings of the 30th Annual International {ACM} {SIGIR}
                  Conference on Research and Development in Information Retrieval, Amsterdam,
                  The Netherlands, July 23-27, 2007},
  pages        = {391--398},
  publisher    = {{ACM}},
  year         = {2007},
  url          = {https://doi.org/10.1145/1277741.1277809},
  doi          = {10.1145/1277741.1277809},
  timestamp    = {Sun, 02 Oct 2022 16:15:17 +0200},
  biburl       = {https://dblp.org/rec/conf/sigir/XuL07.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{listwiseSupportVector2007,
  author       = {Yisong Yue and
                  Thomas Finley and
                  Filip Radlinski and
                  Thorsten Joachims},
  editor       = {Wessel Kraaij and
                  Arjen P. de Vries and
                  Charles L. A. Clarke and
                  Norbert Fuhr and
                  Noriko Kando},
  title        = {A support vector method for optimizing average precision},
  booktitle    = {{SIGIR} 2007: Proceedings of the 30th Annual International {ACM} {SIGIR}
                  Conference on Research and Development in Information Retrieval, Amsterdam,
                  The Netherlands, July 23-27, 2007},
  pages        = {271--278},
  publisher    = {{ACM}},
  year         = {2007},
  url          = {https://doi.org/10.1145/1277741.1277790},
  doi          = {10.1145/1277741.1277790},
  timestamp    = {Tue, 06 Nov 2018 11:07:24 +0100},
  biburl       = {https://dblp.org/rec/conf/sigir/YueFRJ07.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{listwiseSoftRank2008,
  author       = {Michael J. Taylor and
                  John Guiver and
                  Stephen Robertson and
                  Tom Minka},
  editor       = {Marc Najork and
                  Andrei Z. Broder and
                  Soumen Chakrabarti},
  title        = {SoftRank: optimizing non-smooth rank metrics},
  booktitle    = {Proceedings of the International Conference on Web Search and Web
                  Data Mining, {WSDM} 2008, Palo Alto, California, USA, February 11-12,
                  2008},
  pages        = {77--86},
  publisher    = {{ACM}},
  year         = {2008},
  url          = {https://doi.org/10.1145/1341531.1341544},
  doi          = {10.1145/1341531.1341544},
  timestamp    = {Thu, 14 Oct 2021 09:49:09 +0200},
  biburl       = {https://dblp.org/rec/conf/wsdm/TaylorGRM08.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{letor4Dataset,
  author       = {Tao Qin and
                  Tie{-}Yan Liu},
  title        = {Introducing {LETOR} 4.0 Datasets},
  journal      = {CoRR},
  volume       = {abs/1306.2597},
  year         = {2013},
  url          = {http://arxiv.org/abs/1306.2597},
  eprinttype    = {arXiv},
  eprint       = {1306.2597},
  timestamp    = {Mon, 13 Aug 2018 16:48:46 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/QinL13.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{GradVaccine2021,
  author       = {Zirui Wang and
                  Yulia Tsvetkov and
                  Orhan Firat and
                  Yuan Cao},
  title        = {Gradient Vaccine: Investigating and Improving Multi-task Optimization
                  in Massively Multilingual Models},
  booktitle    = {9th International Conference on Learning Representations, {ICLR} 2021,
                  Virtual Event, Austria, May 3-7, 2021},
  publisher    = {OpenReview.net},
  year         = {2021},
  url          = {https://openreview.net/forum?id=F1vEjWK-lH\_},
  timestamp    = {Wed, 23 Jun 2021 17:36:39 +0200},
  biburl       = {https://dblp.org/rec/conf/iclr/WangTF021.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{GradNorm2018,
  author       = {Zhao Chen and
                  Vijay Badrinarayanan and
                  Chen{-}Yu Lee and
                  Andrew Rabinovich},
  editor       = {Jennifer G. Dy and
                  Andreas Krause},
  title        = {GradNorm: Gradient Normalization for Adaptive Loss Balancing in Deep
                  Multitask Networks},
  booktitle    = {Proceedings of the 35th International Conference on Machine Learning,
                  {ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July
                  10-15, 2018},
  series       = {Proceedings of Machine Learning Research},
  volume       = {80},
  pages        = {793--802},
  publisher    = {{PMLR}},
  year         = {2018},
  url          = {http://proceedings.mlr.press/v80/chen18a.html},
  timestamp    = {Fri, 13 Sep 2019 14:28:39 +0200},
  biburl       = {https://dblp.org/rec/conf/icml/ChenBLR18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{uncertaintyWeight2018,
  author       = {Alex Kendall and
                  Yarin Gal and
                  Roberto Cipolla},
  title        = {Multi-Task Learning Using Uncertainty to Weigh Losses for Scene Geometry
                  and Semantics},
  booktitle    = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
                  {CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages        = {7482--7491},
  publisher    = {Computer Vision Foundation / {IEEE} Computer Society},
  year         = {2018},
  url          = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Kendall\_Multi-Task\_Learning\_Using\_CVPR\_2018\_paper.html},
  doi          = {10.1109/CVPR.2018.00781},
  timestamp    = {Fri, 24 Mar 2023 00:02:52 +0100},
  biburl       = {https://dblp.org/rec/conf/cvpr/KendallGC18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pcgrad2020,
  author       = {Tianhe Yu and
                  Saurabh Kumar and
                  Abhishek Gupta and
                  Sergey Levine and
                  Karol Hausman and
                  Chelsea Finn},
  editor       = {Hugo Larochelle and
                  Marc'Aurelio Ranzato and
                  Raia Hadsell and
                  Maria{-}Florina Balcan and
                  Hsuan{-}Tien Lin},
  title        = {Gradient Surgery for Multi-Task Learning},
  booktitle    = {Advances in Neural Information Processing Systems 33: Annual Conference
                  on Neural Information Processing Systems 2020, NeurIPS 2020, December
                  6-12, 2020, virtual},
  year         = {2020},
  url          = {https://proceedings.neurips.cc/paper/2020/hash/3fe78a8acf5fda99de95303940a2420c-Abstract.html},
  timestamp    = {Thu, 24 Mar 2022 15:38:20 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/YuK0LHF20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{alignedMTL2023,
  author       = {Dmitry Senushkin and
                  Nikolay Patakin and
                  Arseny Kuznetsov and
                  Anton Konushin},
  title        = {Independent Component Alignment for Multi-Task Learning},
  booktitle    = {{IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
                  {CVPR} 2023, Vancouver, BC, Canada, June 17-24, 2023},
  pages        = {20083--20093},
  publisher    = {{IEEE}},
  year         = {2023},
  url          = {https://doi.org/10.1109/CVPR52729.2023.01923},
  doi          = {10.1109/CVPR52729.2023.01923},
  timestamp    = {Tue, 29 Aug 2023 15:44:40 +0200},
  biburl       = {https://dblp.org/rec/conf/cvpr/SenushkinPK023.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{MoCo2023,
  author       = {Heshan Devaka Fernando and
                  Han Shen and
                  Miao Liu and
                  Subhajit Chaudhury and
                  Keerthiram Murugesan and
                  Tianyi Chen},
  title        = {Mitigating Gradient Bias in Multi-objective Learning: {A} Provably
                  Convergent Approach},
  booktitle    = {The Eleventh International Conference on Learning Representations,
                  {ICLR} 2023, Kigali, Rwanda, May 1-5, 2023},
  publisher    = {OpenReview.net},
  year         = {2023},
  url          = {https://openreview.net/pdf?id=dLAYGdKTi2},
  timestamp    = {Fri, 30 Jun 2023 14:55:52 +0200},
  biburl       = {https://dblp.org/rec/conf/iclr/FernandoSLCMC23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{metaBalance2022,
  author       = {Yun He and
                  Xue Feng and
                  Cheng Cheng and
                  Geng Ji and
                  Yunsong Guo and
                  James Caverlee},
  editor       = {Fr{\'{e}}d{\'{e}}rique Laforest and
                  Rapha{\"{e}}l Troncy and
                  Elena Simperl and
                  Deepak Agarwal and
                  Aristides Gionis and
                  Ivan Herman and
                  Lionel M{\'{e}}dini},
  title        = {MetaBalance: Improving Multi-Task Recommendations via Adapting Gradient
                  Magnitudes of Auxiliary Tasks},
  booktitle    = {{WWW} '22: The {ACM} Web Conference 2022, Virtual Event, Lyon, France,
                  April 25 - 29, 2022},
  pages        = {2205--2215},
  publisher    = {{ACM}},
  year         = {2022},
  url          = {https://doi.org/10.1145/3485447.3512093},
  doi          = {10.1145/3485447.3512093},
  timestamp    = {Thu, 23 Jun 2022 19:54:34 +0200},
  biburl       = {https://dblp.org/rec/conf/www/0001FC0GC22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{RankFlow2022,
  author       = {Jiarui Qin and
                  Jiachen Zhu and
                  Bo Chen and
                  Zhirong Liu and
                  Weiwen Liu and
                  Ruiming Tang and
                  Rui Zhang and
                  Yong Yu and
                  Weinan Zhang},
  editor       = {Enrique Amig{\'{o}} and
                  Pablo Castells and
                  Julio Gonzalo and
                  Ben Carterette and
                  J. Shane Culpepper and
                  Gabriella Kazai},
  title        = {RankFlow: Joint Optimization of Multi-Stage Cascade Ranking Systems
                  as Flows},
  booktitle    = {{SIGIR} '22: The 45th International {ACM} {SIGIR} Conference on Research
                  and Development in Information Retrieval, Madrid, Spain, July 11 -
                  15, 2022},
  pages        = {814--824},
  publisher    = {{ACM}},
  year         = {2022},
  url          = {https://doi.org/10.1145/3477495.3532050},
  doi          = {10.1145/3477495.3532050},
  timestamp    = {Sun, 20 Aug 2023 13:39:46 +0200},
  biburl       = {https://dblp.org/rec/conf/sigir/QinZ0LLTZY022.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{cascadeRanking2011,
  author       = {Lidan Wang and
                  Jimmy Lin and
                  Donald Metzler},
  editor       = {Wei{-}Ying Ma and
                  Jian{-}Yun Nie and
                  Ricardo Baeza{-}Yates and
                  Tat{-}Seng Chua and
                  W. Bruce Croft},
  title        = {A cascade ranking model for efficient ranked retrieval},
  booktitle    = {Proceeding of the 34th International {ACM} {SIGIR} Conference on Research
                  and Development in Information Retrieval, {SIGIR} 2011, Beijing, China,
                  July 25-29, 2011},
  pages        = {105--114},
  publisher    = {{ACM}},
  year         = {2011},
  url          = {https://doi.org/10.1145/2009916.2009934},
  doi          = {10.1145/2009916.2009934},
  timestamp    = {Fri, 27 Aug 2021 11:12:59 +0200},
  biburl       = {https://dblp.org/rec/conf/sigir/WangLM11.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{cascade_ranking_retrieval,
  author       = {Lidan Wang and
                  Jimmy Lin and
                  Donald Metzler},
  editor       = {Wei{-}Ying Ma and
                  Jian{-}Yun Nie and
                  Ricardo Baeza{-}Yates and
                  Tat{-}Seng Chua and
                  W. Bruce Croft},
  title        = {A cascade ranking model for efficient ranked retrieval},
  booktitle    = {Proceeding of the 34th International {ACM} {SIGIR} Conference on Research
                  and Development in Information Retrieval, {SIGIR} 2011, Beijing, China,
                  July 25-29, 2011},
  pages        = {105--114},
  publisher    = {{ACM}},
  year         = {2011},
  url          = {https://doi.org/10.1145/2009916.2009934},
  doi          = {10.1145/2009916.2009934},
  timestamp    = {Fri, 27 Aug 2021 11:12:59 +0200},
  biburl       = {https://dblp.org/rec/conf/sigir/WangLM11.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{efficient_cost_aware_cascade_ranking,
  author       = {Ruey{-}Cheng Chen and
                  Luke Gallagher and
                  Roi Blanco and
                  J. Shane Culpepper},
  editor       = {Noriko Kando and
                  Tetsuya Sakai and
                  Hideo Joho and
                  Hang Li and
                  Arjen P. de Vries and
                  Ryen W. White},
  title        = {Efficient Cost-Aware Cascade Ranking in Multi-Stage Retrieval},
  booktitle    = {Proceedings of the 40th International {ACM} {SIGIR} Conference on
                  Research and Development in Information Retrieval, Shinjuku, Tokyo,
                  Japan, August 7-11, 2017},
  pages        = {445--454},
  publisher    = {{ACM}},
  year         = {2017},
  url          = {https://doi.org/10.1145/3077136.3080819},
  doi          = {10.1145/3077136.3080819},
  timestamp    = {Tue, 06 Nov 2018 11:07:23 +0100},
  biburl       = {https://dblp.org/rec/conf/sigir/ChenGBC17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{cascade_document_ranking,
  author       = {Zhen Li and
                  Chongyang Tao and
                  Jiazhan Feng and
                  Tao Shen and
                  Dongyan Zhao and
                  Xiubo Geng and
                  Daxin Jiang},
  editor       = {Anna Rogers and
                  Jordan L. Boyd{-}Graber and
                  Naoaki Okazaki},
  title        = {{FAA:} Fine-grained Attention Alignment for Cascade Document Ranking},
  booktitle    = {Proceedings of the 61st Annual Meeting of the Association for Computational
                  Linguistics (Volume 1: Long Papers), {ACL} 2023, Toronto, Canada,
                  July 9-14, 2023},
  pages        = {1688--1700},
  publisher    = {Association for Computational Linguistics},
  year         = {2023},
  url          = {https://doi.org/10.18653/v1/2023.acl-long.94},
  doi          = {10.18653/v1/2023.acl-long.94},
  timestamp    = {Thu, 10 Aug 2023 12:35:57 +0200},
  biburl       = {https://dblp.org/rec/conf/acl/LiTF00GJ23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{cascade_ranking_linkedin,
  author       = {Zimeng Yang and
                  Song Yan and
                  Abhimanyu Lad and
                  Xiaowei Liu and
                  Weiwei Guo},
  editor       = {Gianluca Demartini and
                  Guido Zuccon and
                  J. Shane Culpepper and
                  Zi Huang and
                  Hanghang Tong},
  title        = {Cascaded Deep Neural Ranking Models in LinkedIn People Search},
  booktitle    = {{CIKM} '21: The 30th {ACM} International Conference on Information
                  and Knowledge Management, Virtual Event, Queensland, Australia, November
                  1 - 5, 2021},
  pages        = {4312--4320},
  publisher    = {{ACM}},
  year         = {2021},
  url          = {https://doi.org/10.1145/3459637.3481899},
  doi          = {10.1145/3459637.3481899},
  timestamp    = {Tue, 16 Aug 2022 23:04:38 +0200},
  biburl       = {https://dblp.org/rec/conf/cikm/YangYLLG21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{joint_optimization_cascade_ranking_models,
  author       = {Luke Gallagher and
                  Ruey{-}Cheng Chen and
                  Roi Blanco and
                  J. Shane Culpepper},
  editor       = {J. Shane Culpepper and
                  Alistair Moffat and
                  Paul N. Bennett and
                  Kristina Lerman},
  title        = {Joint Optimization of Cascade Ranking Models},
  booktitle    = {Proceedings of the Twelfth {ACM} International Conference on Web Search
                  and Data Mining, {WSDM} 2019, Melbourne, VIC, Australia, February
                  11-15, 2019},
  pages        = {15--23},
  publisher    = {{ACM}},
  year         = {2019},
  url          = {https://doi.org/10.1145/3289600.3290986},
  doi          = {10.1145/3289600.3290986},
  timestamp    = {Sat, 30 May 2020 20:02:29 +0200},
  biburl       = {https://dblp.org/rec/conf/wsdm/GallagherCBC19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{cooperative_retriever_ranker,
  author       = {Xu Huang and
                  Defu Lian and
                  Jin Chen and
                  Liu Zheng and
                  Xing Xie and
                  Enhong Chen},
  editor       = {Ying Ding and
                  Jie Tang and
                  Juan F. Sequeda and
                  Lora Aroyo and
                  Carlos Castillo and
                  Geert{-}Jan Houben},
  title        = {Cooperative Retriever and Ranker in Deep Recommenders},
  booktitle    = {Proceedings of the {ACM} Web Conference 2023, {WWW} 2023, Austin,
                  TX, USA, 30 April 2023 - 4 May 2023},
  pages        = {1150--1161},
  publisher    = {{ACM}},
  year         = {2023},
  url          = {https://doi.org/10.1145/3543507.3583422},
  doi          = {10.1145/3543507.3583422},
  timestamp    = {Mon, 28 Aug 2023 21:17:10 +0200},
  biburl       = {https://dblp.org/rec/conf/www/HuangLCZ0C23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{ndcg_theoretical,
  author       = {Yining Wang and
                  Liwei Wang and
                  Yuanzhi Li and
                  Di He and
                  Tie{-}Yan Liu},
  title        = {A Theoretical Analysis of {NDCG} Type Ranking Measures},
  booktitle    = {{COLT} 2013 - The 26th Annual Conference on Learning Theory, June
                  12-14, 2013, Princeton University, NJ, {USA}},
  series       = {{JMLR} Workshop and Conference Proceedings},
  volume       = {30},
  pages        = {25--54},
  publisher    = {JMLR.org},
  year         = {2013},
  url          = {http://proceedings.mlr.press/v30/Wang13.html},
  timestamp    = {Wed, 17 Feb 2021 09:07:04 +0100},
  biburl       = {https://dblp.org/rec/conf/colt/WangWLHL13.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@article{multitask_survey,
  author       = {Yu Zhang and
                  Qiang Yang},
  title        = {A Survey on Multi-Task Learning},
  journal      = {{IEEE} Trans. Knowl. Data Eng.},
  volume       = {34},
  number       = {12},
  pages        = {5586--5609},
  year         = {2022},
  url          = {https://doi.org/10.1109/TKDE.2021.3070203},
  doi          = {10.1109/TKDE.2021.3070203},
  timestamp    = {Fri, 23 Dec 2022 13:38:57 +0100},
  biburl       = {https://dblp.org/rec/journals/tkde/ZhangY22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{microsoft_wmt2021,
  author       = {Jian Yang and
                  Shuming Ma and
                  Haoyang Huang and
                  Dongdong Zhang and
                  Li Dong and
                  Shaohan Huang and
                  Alexandre Muzio and
                  Saksham Singhal and
                  Hany Hassan and
                  Xia Song and
                  Furu Wei},
  title        = {Multilingual Machine Translation Systems from Microsoft for {WMT21}
                  Shared Task},
  booktitle    = {Proceedings of the Sixth Conference on Machine Translation, WMT@EMNLP
                  2021, Online Event, November 10-11, 2021},
  pages        = {446--455},
  publisher    = {Association for Computational Linguistics},
  year         = {2021},
  url          = {https://aclanthology.org/2021.wmt-1.54},
  timestamp    = {Wed, 19 Jan 2022 17:10:33 +0100},
  biburl       = {https://dblp.org/rec/conf/wmt/YangMH00HMSHSW21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{hltmt,
  author       = {Jian Yang and
                  Yuwei Yin and
                  Shuming Ma and
                  Dongdong Zhang and
                  Zhoujun Li and
                  Furu Wei},
  title        = {High-resource Language-specific Training for Multilingual Neural Machine
                  Translation},
  booktitle    = {Proceedings of the Thirty-First International Joint Conference on
                  Artificial Intelligence, {IJCAI} 2022, Vienna, Austria, 23-29 July
                  2022},
  pages        = {4461--4467},
  publisher    = {ijcai.org},
  year         = {2022},
  url          = {https://doi.org/10.24963/ijcai.2022/619},
  doi          = {10.24963/ijcai.2022/619},
  timestamp    = {Tue, 21 Mar 2023 20:58:22 +0100},
  biburl       = {https://dblp.org/rec/conf/ijcai/YangYM00W22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{biqa_mtl,
  author       = {Weixia Zhang and
                  Guangtao Zhai and
                  Ying Wei and
                  Xiaokang Yang and
                  Kede Ma},
  title        = {Blind Image Quality Assessment via Vision-Language Correspondence:
                  {A} Multitask Learning Perspective},
  booktitle    = {{IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
                  {CVPR} 2023, Vancouver, BC, Canada, June 17-24, 2023},
  pages        = {14071--14081},
  publisher    = {{IEEE}},
  year         = {2023},
  url          = {https://doi.org/10.1109/CVPR52729.2023.01352},
  doi          = {10.1109/CVPR52729.2023.01352},
  timestamp    = {Sun, 03 Sep 2023 19:31:37 +0200},
  biburl       = {https://dblp.org/rec/conf/cvpr/ZhangZWYM23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{minecraft_mtl,
  author       = {Ingmar Kanitscheider and
                  Joost Huizinga and
                  David Farhi and
                  William Hebgen Guss and
                  Brandon Houghton and
                  Raul Sampedro and
                  Peter Zhokhov and
                  Bowen Baker and
                  Adrien Ecoffet and
                  Jie Tang and
                  Oleg Klimov and
                  Jeff Clune},
  title        = {Multi-task curriculum learning in a complex, visual, hard-exploration
                  domain: Minecraft},
  journal      = {CoRR},
  volume       = {abs/2106.14876},
  year         = {2021},
  url          = {https://arxiv.org/abs/2106.14876},
  eprinttype    = {arXiv},
  eprint       = {2106.14876},
  timestamp    = {Wed, 30 Jun 2021 16:14:10 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2106-14876.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{rank_rate_mtl,
  author       = {Guy Hadash and
                  Oren Sar Shalom and
                  Rita Osadchy},
  title        = {Rank and rate: multi-task learning for recommender systems},
  booktitle    = {Proceedings of the 12th {ACM} Conference on Recommender Systems, RecSys
                  2018, Vancouver, BC, Canada, October 2-7, 2018},
  pages        = {451--454},
  publisher    = {{ACM}},
  year         = {2018},
  url          = {https://doi.org/10.1145/3240323.3240406},
  doi          = {10.1145/3240323.3240406},
  timestamp    = {Wed, 21 Nov 2018 12:44:02 +0100},
  biburl       = {https://dblp.org/rec/conf/recsys/HadashSO18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{better_ranking_consistency_mtl,
  author       = {Xuewei Wang and
                  Qiang Jin and
                  Shengyu Huang and
                  Min Zhang and
                  Xi Liu and
                  Zhengli Zhao and
                  Yukun Chen and
                  Zhengyu Zhang and
                  Jiyan Yang and
                  Ellie Wen and
                  Sagar Chordia and
                  Wenlin Chen and
                  Qin Huang},
  title        = {Towards the Better Ranking Consistency: {A} Multi-task Learning Framework
                  for Early Stage Ads Ranking},
  journal      = {CoRR},
  volume       = {abs/2307.11096},
  year         = {2023},
  url          = {https://doi.org/10.48550/arXiv.2307.11096},
  doi          = {10.48550/arXiv.2307.11096},
  eprinttype    = {arXiv},
  eprint       = {2307.11096},
  timestamp    = {Wed, 26 Jul 2023 15:34:01 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2307-11096.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{istellaDataset,
  author       = {Domenico Dato and
                  Claudio Lucchese and
                  Franco Maria Nardini and
                  Salvatore Orlando and
                  Raffaele Perego and
                  Nicola Tonellotto and
                  Rossano Venturini},
  title        = {Fast Ranking with Additive Ensembles of Oblivious and Non-Oblivious
                  Regression Trees},
  journal      = {{ACM} Trans. Inf. Syst.},
  volume       = {35},
  number       = {2},
  pages        = {15:1--15:31},
  year         = {2016},
  url          = {https://doi.org/10.1145/2987380},
  doi          = {10.1145/2987380},
  timestamp    = {Sun, 02 Oct 2022 15:51:53 +0200},
  biburl       = {https://dblp.org/rec/journals/tois/DatoLNOPTV16.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{diffsort2022,
  author       = {Felix Petersen and
                  Christian Borgelt and
                  Hilde Kuehne and
                  Oliver Deussen},
  title        = {Monotonic Differentiable Sorting Networks},
  booktitle    = {The Tenth International Conference on Learning Representations, {ICLR}
                  2022, Virtual Event, April 25-29, 2022},
  publisher    = {OpenReview.net},
  year         = {2022},
  url          = {https://openreview.net/forum?id=IcUWShptD7d},
  timestamp    = {Sat, 20 Aug 2022 01:15:42 +0200},
  biburl       = {https://dblp.org/rec/conf/iclr/PetersenBKD22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{diffsort2021,
  author       = {Felix Petersen and
                  Christian Borgelt and
                  Hilde Kuehne and
                  Oliver Deussen},
  title        = {Differentiable Sorting Networks for Scalable Sorting and Ranking Supervision},
  booktitle    = {Proceedings of the 38th International Conference on Machine Learning,
                  {ICML} 2021, 18-24 July 2021, Virtual Event},
  series       = {Proceedings of Machine Learning Research},
  volume       = {139},
  pages        = {8546--8555},
  publisher    = {{PMLR}},
  year         = {2021},
  url          = {http://proceedings.mlr.press/v139/petersen21a.html},
  timestamp    = {Thu, 14 Oct 2021 10:33:05 +0200},
  biburl       = {https://dblp.org/rec/conf/icml/PetersenBKD21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@article{deep_multiview_rank,
  author       = {Guanqun Cao and
                  Alexandros Iosifidis and
                  Moncef Gabbouj and
                  Vijay Raghavan and
                  Raju Gottumukkala},
  title        = {Deep Multi-View Learning to Rank},
  journal      = {{IEEE} Trans. Knowl. Data Eng.},
  volume       = {33},
  number       = {4},
  pages        = {1426--1438},
  year         = {2021},
  url          = {https://doi.org/10.1109/TKDE.2019.2942590},
  doi          = {10.1109/TKDE.2019.2942590},
  timestamp    = {Wed, 07 Apr 2021 15:58:40 +0200},
  biburl       = {https://dblp.org/rec/journals/tkde/CaoIGRG21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ModelLog1p2021,
title={Are Neural Rankers still Outperformed by Gradient Boosted Decision Trees?},
author={Zhen Qin and Le Yan and Honglei Zhuang and Yi Tay and Rama Kumar Pasumarthi and Xuanhui Wang and Michael Bendersky and Marc Najork},
booktitle={International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=Ut1vF_q_vC}
}

@inproceedings{approxNdcgDnn2019,
  title={Revisiting approximate metric optimization in the age of deep neural networks},
  author={Bruch, Sebastian and Zoghi, Masrour and Bendersky, Michael and Najork, Marc},
  booktitle={Proceedings of the 42nd international ACM SIGIR conference on research and development in information retrieval},
  pages={1241--1244},
  year={2019}
}

@inproceedings{lambda@k2022,
author = {Jagerman, Rolf and Qin, Zhen and Wang, Xuanhui and Bendersky, Michael and Najork, Marc},
title = {On Optimizing Top-K Metrics for Neural Ranking Models},
year = {2022},
isbn = {9781450387323},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3477495.3531849},
doi = {10.1145/3477495.3531849},
pages = {2303–2307},
numpages = {5},
keywords = {ranking metric optimization, learning to rank, lambdaloss},
location = {Madrid, Spain},
series = {SIGIR '22}
}

@inproceedings{selu2017,
  author       = {G{\"{u}}nter Klambauer and
                  Thomas Unterthiner and
                  Andreas Mayr and
                  Sepp Hochreiter},
  title        = {Self-Normalizing Neural Networks},
  booktitle    = {Advances in Neural Information Processing Systems 30: Annual Conference
                  on Neural Information Processing Systems 2017, December 4-9, 2017,
                  Long Beach, CA, {USA}},
  pages        = {971--980},
  year         = {2017},
  url          = {https://proceedings.neurips.cc/paper/2017/hash/5d44ee6f2c3f71b73125876103c8f6c4-Abstract.html},
  timestamp    = {Thu, 21 Jan 2021 17:36:47 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/KlambauerUMH17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{optimalTransport2019,
  author       = {Marco Cuturi and
                  Olivier Teboul and
                  Jean{-}Philippe Vert},
  title        = {Differentiable Ranking and Sorting using Optimal Transport},
  booktitle    = {Advances in Neural Information Processing Systems 32: Annual Conference
                  on Neural Information Processing Systems 2019, NeurIPS 2019, December
                  8-14, 2019, Vancouver, BC, Canada},
  pages        = {6858--6868},
  year         = {2019},
  url          = {https://proceedings.neurips.cc/paper/2019/hash/d8c24ca8f23c562a5600876ca2a550ce-Abstract.html},
  timestamp    = {Mon, 16 May 2022 15:41:51 +0200},
  biburl       = {https://dblp.org/rec/conf/nips/CuturiTV19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{fastSort2020,
  author       = {Mathieu Blondel and
                  Olivier Teboul and
                  Quentin Berthet and
                  Josip Djolonga},
  title        = {Fast Differentiable Sorting and Ranking},
  booktitle    = {Proceedings of the 37th International Conference on Machine Learning,
                  {ICML} 2020, 13-18 July 2020, Virtual Event},
  series       = {Proceedings of Machine Learning Research},
  volume       = {119},
  pages        = {950--959},
  publisher    = {{PMLR}},
  year         = {2020},
  url          = {http://proceedings.mlr.press/v119/blondel20a.html},
  timestamp    = {Tue, 15 Dec 2020 17:40:18 +0100},
  biburl       = {https://dblp.org/rec/conf/icml/BlondelTBD20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{relu2011,
  author       = {Xavier Glorot and
                  Antoine Bordes and
                  Yoshua Bengio},
  title        = {Deep Sparse Rectifier Neural Networks},
  booktitle    = {Proceedings of the Fourteenth International Conference on Artificial
                  Intelligence and Statistics, {AISTATS} 2011, Fort Lauderdale, USA,
                  April 11-13, 2011},
  series       = {{JMLR} Proceedings},
  volume       = {15},
  pages        = {315--323},
  publisher    = {JMLR.org},
  year         = {2011},
  url          = {http://proceedings.mlr.press/v15/glorot11a/glorot11a.pdf},
  timestamp    = {Thu, 14 Oct 2021 09:27:42 +0200},
  biburl       = {https://dblp.org/rec/journals/jmlr/GlorotBB11.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ple2020,
  author       = {Hongyan Tang and
                  Junning Liu and
                  Ming Zhao and
                  Xudong Gong},
  title        = {Progressive Layered Extraction {(PLE):} {A} Novel Multi-Task Learning
                  {(MTL)} Model for Personalized Recommendations},
  booktitle    = {RecSys 2020: Fourteenth {ACM} Conference on Recommender Systems, Virtual
                  Event, Brazil, September 22-26, 2020},
  pages        = {269--278},
  publisher    = {{ACM}},
  year         = {2020},
  url          = {https://doi.org/10.1145/3383313.3412236},
  doi          = {10.1145/3383313.3412236},
  timestamp    = {Thu, 24 Sep 2020 10:19:44 +0200},
  biburl       = {https://dblp.org/rec/conf/recsys/TangLZG20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{star2021,
  author       = {Xiang{-}Rong Sheng and
                  Liqin Zhao and
                  Guorui Zhou and
                  Xinyao Ding and
                  Binding Dai and
                  Qiang Luo and
                  Siran Yang and
                  Jingshan Lv and
                  Chi Zhang and
                  Hongbo Deng and
                  Xiaoqiang Zhu},
  title        = {One Model to Serve All: Star Topology Adaptive Recommender for Multi-Domain
                  {CTR} Prediction},
  booktitle    = {{CIKM} '21: The 30th {ACM} International Conference on Information
                  and Knowledge Management, Virtual Event, Queensland, Australia, November
                  1 - 5, 2021},
  pages        = {4104--4113},
  publisher    = {{ACM}},
  year         = {2021},
  url          = {https://doi.org/10.1145/3459637.3481941},
  doi          = {10.1145/3459637.3481941},
  timestamp    = {Tue, 16 Aug 2022 23:04:38 +0200},
  biburl       = {https://dblp.org/rec/conf/cikm/ShengZZDDLYLZDZ21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}
